Why Did the Chicken Cross the Road? Rephrasing and Analyzing Ambiguous Questions in VQA

Natural language is ambiguous. Resolving ambiguous questions is key to successfully answering them. Focusing on questions about images, we create a dataset of ambiguous examples. We annotate these, grouping answers by the underlying question they address and rephrasing the question for each group to reduce ambiguity. Our analysis reveals a linguistically-aligned ontology of reasons for ambiguity in visual questions. We then develop an English question-generation model which we demonstrate via automatic and human evaluation produces less ambiguous questions. We further show that the question generation objective we use allows the model to integrate answer group information without any direct supervision.

==> long_ontology.tex <==

\paragraph{Property-based}
Property-based examples typically contain questions about objects with multiple properties which can be used to partition the set of possible worlds (to adopt the terminology of \citet{groenendijk.j.1984}, cf. \cref{sec:groenendijk}). 
Different annotators may choose different partition functions; since answers correspond cells in the partition induced by the question, different partition functions may lead to very different answer sets. 
Property-based questions often correspond to ``where'', ``what'', and ``when'' questions, and often feature a form of under-specification, where the question can be edited to include more information about the relevant partition function. 
\begin{itemize}
    \item \textbf{Location (A/L)}: maps to {\tt{ARGM-LOC}} and asks about the location of an object. Answers here typically differ in terms of frame-of-reference, tracking with the observations of \citet{viethen.j.2008}.
    \item \textbf{Time (A/T)}: maps to {\tt{ARGM-TMP}} and asks about the time of an event or the time a picture was taken. Answers often differ in terms of granularity and frame-of-reference (e.g. ``morning'', ``breakfast time'', ``8am''). 
    \item \textbf{Kind (A/K)}: these do not map to PropBank, and ask about what type or kind of something an object is. Answers differ in terms of property class chosen, e.g. ``what type of car'' -> ``white'', ``sedan'', ``fast''. 
\end{itemize}
\paragraph{Dynamic}
Dynamic questions are typically about properties of dynamic objects or events. 
Annotators often disagree on the type of question being asked (e.g. \emph{cause} vs. \emph{purpose}), as well as the underlying question within a type. 
These questions commonly correspond to ``why'' and ``how'' questions. 
\begin{itemize}
    \item \textbf{Cause (A/C)}: maps to {\tt{ARGM-CAU}}. These ask for the cause of an event. Since cause and purpose are often ambiguous \citep{chapman.c.2016} annotators may differ here, and since cause is often under-specified from a static image, annotators may impute different causes. 
    Even when causes are not imputed, annotators often may choose one of multiple causes, or report causes at different levels of granularity. 
    \item \textbf{Purpose (A/P)}: maps to {\tt{ARGM-PRP}}. Purpose questions ask for the purpose of an event, and share their features with the \emph{cause} examples. 
    \item \textbf{Goal (A/G)}: maps to {\tt{ARGM-GOL}}. These ask for the eventual goal (location or person) of an object or event. 
    When the goal is a person, it is often the person who benefits from an action. 
    Goals are often imputed, and can often be ambiguous with direction. 
    \item \textbf{Direction (A/D)}: maps to {\tt{ARGM-DIR}}. Direction questions as for the path being taken by an object. 
    Sources of disagreement include imputation and choosing from multiple options. 
    \item \textbf{Manner (A/N)}: maps to {\tt{ARGM-MNR}} and asks in what manner an event is happening. 
    Manner questions can be ambiguous with cause questions. 
\end{itemize}
\paragraph{Pragmatic/Other}
\begin{itemize}
    \item \textbf{Multiple Options (A/M)}: a common source of disagreement is when annotators are asked to choose one of multiple options. For example, a question like ``what color is X?'' when X has multiple colors will often result in a variety of answers. 
    Here, the ambiguity is with respect to the inferred intent of the questioner; the answerer must infer which option is most salient to the speaker. 
    \item \textbf{Uncertainty (U)}: many examples contain visual uncertainty, especially for questions about events, which are inherently hard to capture in a static image. 
    \item \textbf{Mistakes}: we find two varieties of mistakes, answering mistakes (M/A) and bad questions and images (M/B). 
    Some annotators provide bad or unreasonable answers to questions; at the same time, some questions are nonsensical and some images are extremely low quality, making answering any question about them impossible. 
\end{itemize}

==> syntax_experiment.tex <==
% For the arxiv and future versions, removing the syntax experiment, which will end up in a later paper 

\section{Cause and Purpose Ambiguity}
``Why'' questions in English are often ambiguous between a cause and purpose reading \citep{chapman.c.2016}. 
In other words, a question like ``Why did the chicken cross the road?" can be interpreted as asking for the purpose of the action (e.g. ``to get to the other side'') or as asking for the impetus for the action (e.g. ``because it was afraid of the fox''). 
\citet{chapman.c.2016} examine such questions in English through a syntactic lens, noting that not all English predicates are ambiguous -- for example, ``why did the butter melt'' has a cause reading, but no purpose reading. 
\citeauthor{chapman.c.2016} conclude that for both readings to exist, the predicate must be dynamic and the subject agentive, factors corresponding to a syntactic analysis with two possible positions for ``why'', each resulting in a different reading. 
Our dataset contains 24 questions labeled with ``cause'' and 16 questions labeled as ``purpose''; of these, 11 have both cause and purpose readings. 
Using this data, we can examine to what extent the \citet{chapman.c.2016}'s hypothesis that ambiguity exists only with dynamic predicates and agentive subjects is borne out in real data.

In light of the small amount of data in our dataset, we first collect additional examples of possible ambiguous ``why'' questions. 
Using the annotations labeled as ambiguous from \citet{bhattacharya.n.2019}, we scrape all questions starting with ``why'' and randomly sample 100.
We manually annotate these as non-ambiguous (i.e. having answers which correspond only to a purpose or only a cause reading) or ambiguous (i.e. having answers for both purpose and cause readings) as well as for dynamicity and agency (cf. \cref{append:why} for examples).
$9$ examples were skipped for having poorly-written questions, resulting in $117$ total examples. 

\vspace{-0.5em}
\paragraph{Results and Analysis} 
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/why_count.pdf}
    \vspace{-2.25em}
    \caption{Count of ambiguous and non-ambiguous questions, grouped by predicate dynamicity (+d) and subject agency (+a). Non-dynamic verbs with non-agentive subjects are also ambiguous between purpose and cause.}
    \label{fig:why_counts}
    \vspace{-1em}
\end{figure}

\cref{fig:why_counts} shows the counts of ambiguously and non-ambiguously-interpreted questions, grouped by whether the predicate is dynamic and its subject agentive.
Part of the hypothesis from \citet{chapman.c.2016} is borne out: we do see often see purpose-reason ambiguity in examples with dynamic predicates and agentive subjects.
However, we also see this ambiguity in all other cases; most notably, in the most common case where the predicate is not dynamic and the subject non-agentive. 
Many of these examples are in fact locative-existential questions, which \citet{chapman.c.2016} identify as only having a reason reading. 
Our results show that speakers disagree with this intuition; for example, for the question ``Why are there cushions on the wall?'' some annotators gave clear reasons (e.g. ``someone put them there'') while others gave purpose answers: ``decoration'', ``padding'', ``design''. 
